Connected Autonomous Vehicle Motion Planning with Video Predictions from Smart, Self-Supervised Infrastructure

Connected autonomous vehicles (CAVs) promise to enhance safety, efficiency, and sustainability in urban transportation. However, this is contingent upon a CAV correctly predicting the motion of surrounding agents and planning its own motion safely. Doing so is challenging in complex urban environments due to frequent occlusions and interactions among many agents. One solution is to leverage smart infrastructure to augment a CAV's situational awareness; the present work leverages a recently proposed "Self-Supervised Traffic Advisor" (SSTA) framework of smart sensors that teach themselves to generate and broadcast useful video predictions of road users. In this work, SSTA predictions are modified to predict future occupancy instead of raw video, which reduces the data footprint of broadcast predictions. The resulting predictions are used within a planning framework, demonstrating that this design can effectively aid CAV motion planning. A variety of numerical experiments study the key factors that make SSTA outputs useful for practical CAV planning in crowded urban environments.

==> sections/A1_T2NO_and_T2ND.tex <==
\subsection{Time to Next Occupancy and Time to Next Departure}

Our goal is motion planning using video predictions.
This requires some way to collision check our ego vehicle's motion in sequences of images containing information about other dynamic agents.
We leverage the fact that an SSTA is static, and can thus capture and use background information, to enable two quantities that simplify collision checking: time to next occupancy, and time to next departure.

Suppose the current time is $t = 0$.
Let $\N_{256} = \{0,1,\cdots,255\}$.
Consider a sequence of predicted images $(I_t)_{t=0}^{T}$ with each image in $\N_{256}^{h\times w\times 3}$, and $T \in \N$ as the \textit{prediction horizon}.
Suppose we also have a \textit{background image} $B \in \N_{256}^{h\times w\times 3}$.
Denote indexing into the $(i,j)$\ts{th} pixel of an image $I$ by $I[i,j]$.
Let $\N_n$ denote the set $\{0,\cdots,n\}$.

The \textit{time to next occupancy} (T2NO) is the first time at which a given pixel in the image is predicted to be occupied, which we assess by comparison against the background.
We represent T2NO as an array $O \in \R^{h\times w}$ that can be thought of as a greyscale image.


\SetKw{Break}{break}

\begin{algorithm}[t]
\caption{Time to Next Occupancy / Departure}
\label{alg:compute_T2NO_and_T2ND}
\KwIn{prediction $(I_t)_{t=0}^T$, background $B$, occupancy threshold $\tau_O$, departure threshold $\tau_D$}

$O, D \gets +\infty_{h\times w}$ // preallocate output

\For{$(i,j) \in \N_h\times \N_w$}{
    $t \gets +\infty$
    // assume no occupancy until infinitely far into the future
    
    \For{$t = 0, 1, \cdots, T$}{
        $\delta \gets |I_t[i,j] - B[i,j]|$
        // error between prediction and background at pixel $(i,j)$
        
        \If{$\delta \geq \tau_O$}{
            $O[i,j] \gets t$
            // get smallest $t$ for which prediction differs from background
            
            \Break
        }
    }
    
    \If{$O[i,j] < +\infty$}{
        \For{$t = O[i,j], O[i,j]+1, \cdots, T$}{
            $\delta \gets |I_t[i,j] - B[i,j]|$
            
            \If{$\delta \leq \tau_D$}{
                $D[i,j] \gets t$
                // get smallest $t$ for which prediction is close to background
                
                \Break
            }
        }
    }
}
\KwOut{$O$}
\end{algorithm}

On its own, T2NO does not capture all relevant dynamic information in a scene, because, once a pixel is declared occupied at a time $t$, it is occupied for all future time $t' > t$.
The \textit{time to next departure} (T2ND) alleviates this concern by measuring the first time at which an occupied pixel is \textit{no longer} occupied.
Similar to T2NO, we represent T2ND as an array $D \in \R^{h\times w}$.
We compute both T2NO and T2ND using Alg. \ref{alg:compute_T2NO_and_T2ND}.

By combining T2NO and T2ND, we assess when each pixel will be occupied and then free within the time horizon $T$.
For example, consider a single car passing through pixel $(i,j)$ at 10 m/s, and consider a pixel that corresponds to a $1 \times 1$ m\ts{2} patch of drivable area.
Suppose the T2NO is $2.0$ s, meaning the earliest time at which that car occupies that pixel.
Suppose the car is $5$ m long.
Then the car will completely pass over the pixel in $0.5$ s, meaning that the T2ND at that pixel must be no less than $2.5$ s.
An adjacent pixel in the direction of travel will have $O[i,j] = 2.1$ s, and $D[i,j] = 2.6$ s (assuming the car is predicted to maintain its speed and heading).


One key limitation of this formulation is that it only predicts a single next occupancy/departure.
This may be insufficient in the case where, for example, a car is followed closely by another car such that a single pixel is occupied multiple separate times within the prediction horizon $T$.
In this case, as an extension for future work, we can predict a \textit{list} $L \in \R^{h\times w\times n_L}$ of occupancy and departure times, where $n_L$ is the total number of times to predict.
For example, if our car is followed by another car $0.5$ s behind in the previous example, then this list at our given pixel may be
\begin{align}
    L[i,j] = [2.0, 2.5, 3.0, 3.5],
\end{align}
where the $n_L = 4$ values in the list are alternating occupancy/departure times.
We can generate this data automatically given our predictions $I_t$ and background image $B$, then train a predictor to directly output $L[i,j]$ at each pixel.





\subsection{Collision Checking}

We seek to use an SSTA's predictions for collision checking within a CAV motion planning framework.
First, we explain how to isolate pixels associated with the ego vehicle for a given pose.
Then, we consider collision checking against T2NO/D.


\subsubsection{Masking the Ego Vehicle's Pixels}

Recall that each SSTA outputs a sequence of images $(I_t)_{t=0}^T$, with each $I_t \in \N_{256}^{h\times w \times 3}$.
Before proceeding, we briefly introduce an approach to extracting the pixels in an image corresponding to our ego vehicle's pose (position and heading), which we denote $(x_t,y_t,\theta_t)$ at time $t$.
Suppose the vehicle has a rectangular body of dimensions $l \times d$.
Also suppose that each pixel, with indices $(i,j)$, is associated with a corresponding spatial location $(x_{i,j}, y_{i,j})$.
Let the following maps convert between pixels and spatial coordinates:
\begin{align}
    \code{px2sp}&: (i,j) \mapsto (x_{i,j}, y_{i,j}) \\
    \code{sp2px}&: (x_{i,j}, y_{i,j}) \mapsto (i,j)
\end{align}
Also, note that we can represent the vehicle's body at the state $(x,y,\theta)$ as an array of vertices arranged counterclockwise:
\begin{align}
    V_t \gets \left(\tfrac{1}{2}
        \left[\begin{smallmatrix*}[r]
            \cos\theta_t & -\sin\theta_t\\
            \sin\theta_t & \cos\theta_t
        \end{smallmatrix*}\right]
        \left[\begin{smallmatrix*}[r]
            l & -l & -l & l \\
            d & d & -d & -d
        \end{smallmatrix*}\right]\right) +
        \left[\begin{smallmatrix}
            x_t \\ y_t
        \end{smallmatrix}\right].
\end{align}
Recall that our images $I_t$ are of dimension $h \times w \times 3$.
We thus create a mask for the given vehicle pose:
\begin{align}
    P_t &\gets \code{sp2px}(V_t) \\
    P_t &\gets \code{fillPoly}(\zeros_{h \times w \times 3},\ P_t), \\
    M_t &\gets P_t = (255,255,255),\label{eq:vehicle_mask}
\end{align}
where $P_t$ is used as an intermediate array.
The second line fills in a polygon defined by the (pixel coordinate) vertices $V_M$, into a black image ($\zeros_{h \times w \times 3}$), so $P_t \in \N_{256}^{h\times w\times 3}$.
Note, \code{fillPoly} is available in OpenCV \cite{opencv_library}, and we assume the default fill color is white, or $(255,255,255)$.
The last line creates the mask $M_t \in \{0,1\}^{h\times w}$ (i.e., a boolean array) which is \code{true} for every entry (i.e., pixel) that is white, thereby identifying the pixels corresponding to our vehicle's pose.

\subsubsection{Checking Against T2NO/D}
This collision check is nearly identical to checking against pixels directly.
In particular, for each time step $t$, we check:
\begin{align}
    M_t &\gets t \cdot M_t \\
    \code{chk}_t & \gets \code{any}\left(M_t \geq O\ \&\ M_t \leq D \right)
\end{align}
The first line converts the boolean mask $M_t$ to a real-valued array, where entries where $M_t$ is \code{true} are set to $t$, and all others are $0$.
Then, we directly check the entries of $M_t \in \R^{h\times w}$ against the T2NO $O \in \R^{h\times w}$ and $D \in \R^{h \times w}$.
If any of the vehicle's occupied pixels (i.e., \code{true} pixels) overlap with the time window created by $O$ and $D$, then $\code{chk}_t$ is \code{true} (i.e., the pose $(x_t,y_t,\theta_t)$ is in collision).

\subsection{Dynamic A*}

\begin{algorithm}
\caption{Classical A* Algorithm}
\label{alg:classical_a_star}
\KwIn{Mark $P(start)$ as $openlist$.}

\While{$openlist \neq \emptyset$}{
    Select the node $P(i)$ from the $openlist$ whose value of evaluation function $F(P(i))$ is smallest.
    
    Mark $P(i)$ as $clostlist$.
    
    \If{$P(i) = P(end)$}{
        \Return "path is found"
    }
    \Else{
        Select the successor node $P_i(j)$ around the node $P(i)$, and calculate $F(P_i(j))$.
        
        \If{$P_i(j)$ \rm{belongs to} $obstacle$ \rm{or} $closelist$ \rm{node}}{
            \textit{continue}
        }
        
        Mark $P_i(j)$ as $openlist$.
        
        \If{$P_i(j)$ \rm{belongs to} $openlist$ \rm{and} $F(P_i(j) < F(P_m(j))$\rm{when} $P(m)$ \rm{was marked as} $closelist$}{
        Set parent node of $P(j)$ as $P(i)$, $F(P(i)) = F(P_i(j))$.
        }
    }
}
\Return "the path cannot be found"
\end{algorithm}

In the classical A-star algorithm the evaluation function $F(P(i))$ of $P(i)$ is defined as Eq.~\ref{equ:a_star_eval_func}:
\begin{equation}
\label{equ:a_star_eval_func}
    F(P(i)) = G(P(i)) + H(P(i)),
\end{equation}
where $G(P(i))$ is the cost of the path from $P(start)$ to $P(i)$, $H(P(i))$ is the cost of the cheapest path from $P(i)$ to $P(end)$. It is worth noting that $H(P(i))$ has several heuristic function forms, such as Manhattan distance, Euclidean distance, diagonal distance, etc. Different heuristic functions have an effect on the search accuracy and rate of the A-star algorithm. In this article, Euclidean distance heuristic functions are used in order to unify the calculations.
\subsection{Cost-aware A* Algorithm}
\subsection{Dynamic A* Algorithm}
\textit{The difference between dynamic A* and D*?}

The searching process of the A-star algorithm for static obstacles is similar to a dynamic window method~\cite{4209377,he2022dynamic}, except that the window becomes eight points around node $P(i)$, and the information about these obstacles do not change over time, i.e., the obstacles are all static. The classical A-star algorithm can only avoid static obstacles. Avoiding dynamic obstacles does not mean that the trajectory of object and the trajectories of the dynamic obstacles cannot be intersected, i.e., reaching the same location at different times is allowed. If the generated path is given the attribute of time, the collision avoiding with dynamic obstacles can be realized in time–space dimension. In the previous analysis, it is difficult for a car to continuously accelerate or decelerate or even stop during navigation. Therefore it is important to generate a path that can avoid dynamic obstacles even if the car is assumed to travel at a uniform speed. Considering that A-star algorithm is searching based on the current node $P(i)$, we only need to determine the time period $T_c$ it takes to travel from the starting point $P(start)$ to the current node $P(i)$. The core idea of the dynamic updating mechanism is to bring the current node $P(i)$ and the starting point $P(start)$ to a subroutine called “findparent”, whose pseudo-code is shown in Algorithm~\ref{alg:a_star_findparent}.
\begin{algorithm}
\caption{findParent$(P(i), P(start))$}
\label{alg:a_star_findparent}
$T_c = 0$

\While{$P(i) \neq P(start)$}{
    Find the parent node $P(i-1)$ of the $P(i)$.
    
    $T_c=T_c + cost\ time$ from $P(i-1)$ to $P(i)$.
    
    $P(i) = P(i-1)$
}
\Return time period $T_c$
\end{algorithm}

\begin{algorithm}
\caption{Dynamic A* Algorithm}
\label{alg:dynamic_a_star}
\KwIn{Mark $P(start)$ as $openlist$.}

\While{$openlist \neq \emptyset$}{
    Select the node $P(i)$ from the $openlist$ whose value of evaluation function $F(P(i))$ is smallest.
    
    Mark $P(i)$ as $clostlist$.
    
    \If{$P(i) = P(end)$}{
        \Return "path is found"
    }
    \Else{
        $T_c = \rm{findParent}(P(i), P(start))$
        
        Sampling the trajetory of the $n$ known dynamic obstacles to get its $T_c$ position $D_n(T_c)$.
        
        \If{$D_n(T_c)$ \rm{does not belong to} $openlist$}{
            Mark $D_n(T_c)$ as $closelist$.
        }
        
        Select the successor node $P_i(j)$ around the node $P(i)$, and calculate $F(P_i(j))$.
        
        \If{$P_i(j)$ \rm{belongs to} $obstacle$ \rm{or} $closelist$ \rm{node}}{
            \textit{continue}
        }
        
        Mark $P_i(j)$ as $openlist$.
        
        \If{$P_i(j)$ \rm{belongs to} $openlist$ \rm{and} $F(P_i(j) < F(P_m(j))$\rm{when} $P(m)$ \rm{was marked as} $closelist$}{
        Set parent node of $P(j)$ as $P(i)$, $F(P(i)) = F(P_i(j))$.
        }
        
        \If{$D_n(T_c)$ \rm{does not belong to} $openlist$}{
        Remove $D_n(T_c)$ from $closelist$.
        }
    }
}
\Return "the path cannot be found"
\end{algorithm}


